Dual-domain Adaptation Networks for Realistic Image Super-resolution

Realistic image super-resolution (SR) focuses on transforming real-world low-resolution (LR) images into high-resolution (HR) ones, handling more complex degradation patterns than synthetic SR tasks. This is critical for applications like surveillance, medical imaging, and consumer electronics. However, current methods struggle with limited real-world LR-HR data, impacting the learning of basic image features. Pre-trained SR models from large-scale synthetic datasets offer valuable prior knowledge, which can improve generalization, speed up training, and reduce the need for extensive real-world data in realistic SR tasks. In this paper, we introduce a novel approach, Dual-domain Adaptation Networks, which is able to efficiently adapt pre-trained image SR models from simulated to real-world datasets. To achieve this target, we first set up a spatial-domain adaptation strategy through selectively updating parameters of pre-trained models and employing the low-rank adaptation technique to adjust frozen parameters. Recognizing that image super-resolution involves recovering high-frequency components, we further integrate a frequency domain adaptation branch into the adapted model, which combines the spectral data of the input and the spatial-domain backbone's intermediate features to infer HR frequency maps, enhancing the SR result. Experimental evaluations on public realistic image SR benchmarks, including RealSR, D2CRealSR, and DRealSR, demonstrate the superiority of our proposed method over existing state-of-the-art models. Codes are available at: https://github.com/dummerchen/DAN.

==> sec/tab4-fda.tex <==
% Table generated by Excel2LaTeX from sheet '对比实验'
\begin{table}[htbp]
 \fontsize{8}{8}\selectfont
  \centering
  \caption{Effect of using frequency-domain adaptation. `SDA' is short for space-domain adaptation. }\vspace{-3mm}
    \setlength{\tabcolsep}{1.6mm}{ \begin{tabular}{|c|l|cc|cc|}
    \hline
     \multirow{2}[4]{*}{No.}    &  \multirow{2}[4]{*}{Variants}    & \multicolumn{2}{c|}{4$\times$}   & \multicolumn{2}{c|}{2$\times$}  \bigstrut\\
\cline{3-6}        &  & PSNR  & SSIM   & PSNR  & SSIM   \bigstrut\\
    \hline
    1  & Implementing FDA as SDA & 29.45 & 0.833 & 34.16 & 0.925  \bigstrut\\
    \hline
    %2  & Using FD loss  & 29.60 & 0.834 & 34.28 & 0.927  \bigstrut\\ 
    %\hline
    2 & Ours FDA & 29.65 & 0.835 & 34.30  & 0.927  \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:fda}%
\end{table}%


\iffalse
\begin{table}[htbp]
 \fontsize{7}{8}\selectfont
  \centering
  \caption{Effect of using frequency-domain adaptation. }
    \setlength{\tabcolsep}{.8mm}{ \begin{tabular}{|c|l|ccc|ccc|}
    \hline
     \multirow{2}[4]{*}{No.}    &  \multirow{2}[4]{*}{Variants}    & \multicolumn{3}{c|}{4$\times$}   & \multicolumn{3}{c|}{2$\times$}  \bigstrut\\
\cline{3-8}        &  & PSNR  & SSIM  & LPIPS & PSNR  & SSIM  & LPIPS \bigstrut\\
    \hline
    1  & Replacing FDA with SDA & 29.53 & 0.835 & 0.263 & 34.25 & 0.927 & 0.133 \bigstrut\\
    \hline
    2  & Using FD loss  & 29.58 & 0.834 & 0.266 & 34.32 & 0.928 & 0.133 \bigstrut\\ 
    \hline
    3 & Ours FDA & 29.68 & 0.836 & 0.269 & 34.40  & 0.928 &0.134 \bigstrut\\
    \hline
    \end{tabular}%
    }
  \label{tab:ablation}%
\end{table}%
\fi
